High-Speed Bullet Ejections during the AGB to Planetary Nebula Transition: HST Observations of the Carbon Star, V Hydrae

The well-studied carbon star, V Hya, showing evidence for high-speed, collimated outflows and dense equatorial structures, is a key object in the study of the poorly understood transition of AGB stars into aspherical planetary nebulae. Using the STIS instrument onboard HST, we have obtained high spatial-resolution long-slit optical spectra of V Hya that show high-velocity emission in [SII] and [FeII] lines. Our dataset, spanning three epochs spaced apart by a year during each of two periods (in 2002-2004 and 2011-2013), shows that V Hya ejects high-speed (about 200-250 km/s) bullets once every ~8.5 yr. The ejection axis flip-flops around a roughly eastern direction, both in and perpendicular to the sky-plane, and the radial velocities of the ejecta also vary in concert between low and high values. We propose a model in which the bullet ejection is associated with the periastron passage of a binary companion in an eccentric orbit around V Hya with an orbital period of ~8.5 yr. The flip-flop phenomenon is likely the result of collimated ejection from an accretion disk (produced by gravitational capture of material from the primary) that is warped and precessing, and/or that has a magnetic field that is misaligned with that of the companion or the primary star. We show how a previously observed 17-year period in V Hya's light-cycle can also be explained in our model. Additionally, we describe how the model proposed here can be extended to account for multipolar nebulae.

==> ObsPropIIITable-test.tex <==
%ADD A TABLE FOR FE[II] at 4288.6 A
\scriptsize
%\begin{turnpage}
\begin{table}{p{0.8in}p{0.45in}p{0.45in}p{0.45in}p{1.0in}}
\caption[]{Observational Properties III (Detached \& On-Source Blobs: [FeII] $\lambda$4288.6)}\\
\hline \\[-2ex]
   \multicolumn{1}{l}{\textbf{Epoch}} &
   \multicolumn{1}{l}{\textbf{Slit}} &
   \multicolumn{1}{l}{\textbf{Offset}} &
   \multicolumn{1}{l}{\textbf{$V_P$}} &
   \multicolumn{1}{l}{\textbf{Flux}} \\[0.5ex] 
   \multicolumn{1}{l}{\textbf{(\#) Date}} &
   \multicolumn{1}{l}{\textbf{Name}} &
   \multicolumn{1}{l}{\textbf{arcsec}} &
   \multicolumn{1}{l}{\textbf{\,\kms}} &
   \multicolumn{1}{l}{\textbf{cgs}} \\[0.5ex] 
   \\[-1.8ex]
\endhead
\hline \\[-2ex]
\multicolumn{1}{l}{\textbf{}} &
\multicolumn{1}{l}{\textbf{}} &
\multicolumn{1}{c}{\textbf{Period 1: Detached Blob}} \\[0.5ex] \hline 
\\[-1.8ex]
(1) 2002-01-28  &  $S_{-2w}$  &  -0.185   &  -246     & 1.8e-14  \\
(2) 2002-12-29  &  $S_{-1n}$  &  -0.236    & -220     & 4.5e-14  \\
(3) 2004-01-12  &  $S_{-1n}$  &  -0.338    &  -196    & 4.0e-14   \\
\hline \\[-2ex]
\multicolumn{1}{l}{\textbf{}} &
\multicolumn{1}{l}{\textbf{}} &
\multicolumn{1}{c}{\textbf{Period 2: On-Source Blob}} \\[0.5ex] \hline
\\[-1.8ex]
(4) 2011-07-07  &  $S_{0w}$   & -0.058  &  -166    &  2.8e-14   \\
(5) 2012-07-14  &  $S_{0w}$   &  0.018  &  -195   &  1.9e-13   \\
(6) 2013-07-17  &  $S_{0w}$   & -0.008  &  -163   &  7.8e-14  \\    
\label{obsfe2}
\end{table}
%\end{center} 
\end{turnpage}

